Few-Shot Incremental Learning with Continually Evolved Classifiers

Few-shot class-incremental learning (FSCIL) aims to design machine learning algorithms that can continually learn new concepts from a few data points, without forgetting knowledge of old classes. The difficulty lies in that limited data from new classes not only lead to significant overfitting issues but also exacerbate the notorious catastrophic forgetting problems. Moreover, as training data come in sequence in FSCIL, the learned classifier can only provide discriminative information in individual sessions, while FSCIL requires all classes to be involved for evaluation. In this paper, we address the FSCIL problem from two aspects. First, we adopt a simple but effective decoupled learning strategy of representations and classifiers that only the classifiers are updated in each incremental session, which avoids knowledge forgetting in the representations. By doing so, we demonstrate that a pre-trained backbone plus a non-parametric class mean classifier can beat state-of-the-art methods. Second, to make the classifiers learned on individual sessions applicable to all classes, we propose a Continually Evolved Classifier (CEC) that employs a graph model to propagate context information between classifiers for adaptation. To enable the learning of CEC, we design a pseudo incremental learning paradigm that episodically constructs a pseudo incremental learning task to optimize the graph parameters by sampling data from the base dataset. Experiments on three popular benchmark datasets, including CIFAR100, miniImageNet, and Caltech-USCD Birds-200-2011 (CUB200), show that our method significantly outperforms the baselines and sets new state-of-the-art results with remarkable advantages.

==> emd_introduction.tex <==
\section{Introduction}
Deep Convolutional Neural Networks have made significant breakthroughs in many visual understanding tasks including image classification~\cite{krizhevsky2012imagenet,resnet,simonyan2014very}, object detection~\cite{ren2015faster,he2017mask,redmon2016you}, and semantic segmentation~\cite{lin2017refinenet,chen2018deeplab,fcn}. One crucial reason is the availability of large-scale datasets such as ImageNet~\cite{imagenet} that enable the training of deep models. However, data labeling is expensive, particularly for dense prediction tasks, \eg, semantic segmentation and instance segmentation.
In contrast to machine learning algorithms, humans are able to segment a new concept from the image easily when only seeing a few examples. The gap between humans and machine learning algorithms motivates the study of few-shot learning that aims to learn a model which can be generalized well to new classes with scarce labeled training data.
\begin{figure}[]
\centering
\includegraphics[width=\linewidth]{latex/pipline.pdf}
\caption{Overview of our proposed network for 1-shot segmentation. Our framework consists of a dense comparison module (DCM) and an iterative optimization module (IOM). Given only one annotated training image, our network is able to segment  test images with new classes and iteratively optimize the results.}
\label{fig:pipline}
\vskip -1em
\end{figure}

In this paper, we undertake the task of few-shot semantic segmentation that only uses a few annotated training images to perform segmentation on new classes. Previous work~\cite{shaban2017one,rakelly2018conditional,Dong2018FewShotSS} on this task follows the design of two-branch structure which includes a support branch and a query branch. The support branch aims to extract information from the support set to guide segmentation in the query branch. We also adopt the two-branch design in our framework to solve the few-shot segmentation problem. 

Our network includes a two-branch dense comparison module, in which a shared feature extractor extracts representations from the query set and the support set for comparison. The design of the dense comparison module takes inspiration from metric learning~\cite{relation,snell2017prototypical} on image classification tasks where a distance function evaluates the similarity between images. However, different from image classification where each image has a label, image segmentation needs to make predictions on data with structured representation.
It is difficult to directly apply metric learning to dense prediction problems.  
To solve this, one straightforward approach is to make comparisons between all pairs of pixels. However, there are millions of pixels in an image and comparison of all pixel pairs takes enormous computational cost. Instead, we aim to acquire a global representation from the support image for comparison. 
Here, to only focus on the assigned category, we use global average pooling over the foreground area to filter out irrelevant information. Then the global feature is compared with each location in the query branch, which can be seen as a dense form of the metric learning approach.

Under the few-shot setting, the network should be able to handle new classes that are never seen during training. Thus we aim to mine transferable representations from CNNs for comparison. As is observed in feature visualization literature~\cite{zeiler2014visualizing,yosinski2015understanding}, features in lower layers relate to low-level cues, \eg, edges and colors while features in higher layers relate to object-level concepts such as categories. We focus on middle-level features that may constitute object parts shared by unseen classes. For example, if the CNN learns a feature that relates to \emph{wheel} when the model is trained on the class \emph{car}, such feature may also be useful for feature comparison on new vehicle classes, \eg, \emph{truck} and \emph{bus}. We extract multiple levels of representations in CNNs for dense comparison. 

As there exist variances in appearance within the same category, objects from the same class may only share a few similar features. Dense feature comparison is not enough to guide segmentation of the whole object area. Nevertheless, this gives an important clue of where the object is. In semi-automatic segmentation literature, weak annotations are given for class-agnostic segmentation, \eg, interactive segmentation with click or scribble annotations~\cite{interative,scribble} and instance segmentation with bounding box or extreme point priors~\cite{segevery,extreme}. Transferable knowledge to locate the object region is learned in the training process. Inspired by semi-automatic segmentation tasks, we hope to gradually differentiate the objects from the background given the dense comparison results as priors. We propose an iterative optimization module (IOM) that learns to iteratively refine the predicted results. The refinement is performed in a recurrent form that the dense comparison result and the predicted masks are sent to an IOM for optimization, and the output is sent to the next IOM recurrently. After a few iterations of refinement, our dense comparison module is able to generate fine-grained segmentation maps. Inside each IOM, we adopt residual connections to efficiently incorporate the predicted masks in the last iteration step.  Fig.~\ref{fig:pipline} shows an overview of our network for one-shot segmentation.

Previous methods for $k$-shot segmentation is based on the 1-shot model. They use non-learnable fusion methods to fuse individual 1-shot results, \eg, averaging 1-shot predictions or intermediate features. Instead, we adopt an attention mechanism to effectively fuse information from multiple support examples.

To further reduce the labeling efforts for few-shot segmentation, we explore a new test setting: our model uses the bounding box annotated support set to perform segmentation in the query image. We conduct comprehensive experiments on the PASCAL VOC 2012 dataset and COCO dataset to validate the effectiveness of our network. 
Main contributions of this paper are summarized as follows.
\begin{itemize}
\itemsep -0.1cm 
	\item We develop a novel two-branch dense comparison module which effectively exploits multiple levels of feature representations from CNNs to make dense feature comparison. 
	\item We propose an iterative optimization module to refine predicted results in an iterative manner. The ability of iterative refinement can be generalized to unseen classes with few-shot learning for generating fine-grained maps.
	\item We adopt an attention mechanism to effectively fuse information from multiple support examples in the $k$-shot setting, which outperforms non-learnable fusion methods of 1-shot results. 
	\item We demonstrate that given support set with weak annotations, \ie, bounding boxes, our model can still achieve comparable performance to the result with expensive pixel-level annotated support set, which further reduces the labeling efforts of new classes for few-shot segmentation significantly.
	\item Experiments on the PASCAL VOC 2012 dataset show that our method achieves a mean Intersection-over-Union score of 55.4\% for 1-shot segmentation and 57.1\% for 5-shot segmentation, which significantly outperform state-of-the-art results by 14.6\% and 13.2\%, respectively.
\end{itemize}





